Relation/Entity-Centric Reading Comprehension

Constructing a machine that understands human language is one of the most elusive and long-standing challenges in artificial intelligence. This thesis addresses this challenge through studies of reading comprehension with a focus on understanding entities and their relationships. More specifically, we focus on question answering tasks designed to measure reading comprehension. We focus on entities and relations because they are typically used to represent the semantics of natural language.

==> section/abstruct.tex <==
Constructing a machine that understands human language is one of the most elusive and long-standing challenges in artificial intelligence. This thesis addresses this challenge through studies of reading comprehension with a focus on understanding entities and their relationships. More specifically, we focus on question answering tasks designed to measure reading comprehension. We focus on entities and relations because they are typically used to represent the semantics of natural language.

In Chapter \ref{sec:introduction}, we overview the history of the reading comprehension tasks and various styles of the tasks. We also differentiate the reading comprehension tasks from other question answering tasks. Then, we present entities and their relations in the context of reading comprehension tasks.

In Chapter \ref{sec:work1}, we present an original reading comprehension dataset. We used baseline systems and a sampling approach to control the difficulty of the dataset. As a result, the dataset achieved a high human performance and low machine performance, and the gap indicates the dataset provides questions that requires deep understanding of texts. 
\thispagestyle{plain}

In Chapter \ref{sec:work2}, we analyze neural network models for reading comprehension tasks and show that the vector representations learned in the models can be understood as being composed of a predicate applied to entities.


In Chapter \ref{sec:wikihop}, we apply our findings in Chapter \ref{sec:work2} to another reading comprehension dataset focusing on entities and their relations. We propose a transformer encoder-based model and show that the model achieves the higher development accuracy than other models with a similar number of parameters. 

In Chapter \ref{sec:work3}, we present our work on relation extraction, a task for predicting a relation of two given entities by using text resources. This work focuses on relations occurring in materials science. We target factors for material development and visualizes these factors and their relations in a graph formalism. The particular factors and their relations are extracted from thousands of materials science articles.

Finally, Chapter \ref{sec:thesis_conclusion} concludes the thesis. 



==> section/acknowledgement.tex <==
It has been an honor for me to be advised by Professor David McAllester, who has been giving me his outstanding mentorship, his patience and unconditional support from the first day to the last day of my graduate program. Through him, I also got to understand more about how to think and act as a true academic scientist. I would never have come this far without his guidance and encouragement.

I would also like to thank Professor Kevin Gimpel for his research collaboration which was a new chapter in my Ph.D. A big thanks to Professor Yutaka Sasaki for the insightful discussions and educational supports that we had and his precise and constructive comments on my thesis. I would also like to thank Professor Makoto Miwa for the insightful discussions that helps me in the early days of my Ph.D. research, and his advice for my Ph.D. thesis. I would like to thank Professor Ikumu Watanabe for the great research collaboration and his insightful advice. 

My special thank goes to the late Mr. Tatsuro Toyoda, the found of Toyota Technological Institute. I really appreciate the opportunity to study in Toyota Technological Institute at Chicago and Japan, and it is a great honor for me to be the first student to graduate from both Toyota Technological Institute in the world. 

My deepest gratitude goes to my family for their endless love and support during all these years. I’d like to thank my parents for supporting my decisions throughout all these years.

\newpage
